Pretty-big-step-semantics-based Certified Abstract Interpretation (Preliminary version)

We present a technique for deriving semantic program analyses from a natural semantics specification of the programming language. The technique is based on a particular kind of semantics called pretty-big-step semantics. We present a pretty-big-step semantics of a language with simple objects called O'While and specify a series of instrumentations of the semantics that explicitates the flows of values in a program. This leads to a semantics-based dependency analysis, at the core, e.g., of tainting analysis in software security. The formalization has been realized with the Coq proof assistant.

==> eptcsdata.tex <==
\providecommand{\firstpage}{360}
\providecommand{\publicationstatus}{A. Banerjee, O. Danvy, K.-G. Doh, J. Hatcliff (Eds):\\
David A. Schmidt's 60th Birthday Festschrift\\
EPTCS 129, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.129.23}{10.4204/EPTCS.129.23}}
\pdfoutput=1

